Automating Bibliometric Analysis with Sentence Transformers and Retrieval-Augmented Generation (RAG): A Pilot Study in Semantic and Contextual Search for Customized Literature Characterization for High-Impact Urban Research

Bibliometric analysis is essential for understanding research trends, scope, and impact in urban science, especially in high-impact journals, such Nature Portfolios. However, traditional methods, relying on keyword searches and basic NLP techniques, often fail to uncover valuable insights not explicitly stated in article titles or keywords. These approaches are unable to perform semantic searches and contextual understanding, limiting their effectiveness in classifying topics and characterizing studies. In this paper, we address these limitations by leveraging Generative AI models, specifically transformers and Retrieval-Augmented Generation (RAG), to automate and enhance bibliometric analysis. We developed a technical workflow that integrates a vector database, Sentence Transformers, a Gaussian Mixture Model (GMM), Retrieval Agent, and Large Language Models (LLMs) to enable contextual search, topic ranking, and characterization of research using customized prompt templates. A pilot study analyzing 223 urban science-related articles published in Nature Communications over the past decade highlights the effectiveness of our approach in generating insightful summary statistics on the quality, scope, and characteristics of papers in high-impact journals. This study introduces a new paradigm for enhancing bibliometric analysis and knowledge retrieval in urban research, positioning an AI agent as a powerful tool for advancing research evaluation and understanding.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> contents/000-backup.tex <==
\citep{fijavcko2024using} explores how generative AI can be applied to bibliometric analysis. Specifically, the study focuses on analyzing 10 years of research abstracts presented at the European Resuscitation Congresses (ERC). The researchers used ChatGPT-4 to classify 2,491 abstracts into ERC guideline topics, employing web scraping and the guidelines set by ERC 2021 as a reference. The most frequently discussed topics identified were Basic Life Support, which accounted for 50.1\% of the abstracts, and Adult Advanced Life Support, at 41.5\%. The study highlights the potential of large language models like ChatGPT-4 in categorizing and analyzing scientific literature, identifying key trends, and assessing the co-occurrence between different topics within the ERC literature.

However, the study also faced significant challenges. One of the primary limitations was the potential for misclassification of abstracts by the AI model, although this issue was reported as minimal. Another limitation arose from the data itself; only the titles of abstracts were available for analysis, restricting the depth of insight that could be achieved compared to using full-text abstracts or complete articles. Additionally, the research relied heavily on the capabilities of the AI model and the quality of the available data, emphasizing the difficulties in fully automating bibliometric tasks, particularly when access to comprehensive datasets is limited. Despite these challenges, the study underscores the growing role of AI in enhancing bibliometric methodologies and uncovering trends in scientific research.
 
\citep{weng2022identification} presents a methodology for detecting and visualizing key research topics in scientific publications using advanced machine learning techniques. The researchers employed GPT-3 embeddings and the HDBSCAN clustering algorithm to analyze 593 abstracts related to urban studies and machine learning. By representing the semantic meaning of each abstract with GPT-3 similarity embeddings, the study aimed to group related abstracts through an unsupervised clustering approach. Keywords were extracted from each abstract using the Maximal Marginal Relevance (MMR) algorithm, ensuring that the most representative terms were selected to encapsulate the content of each abstract. The clustering and keyword extraction results were then visualized in an interactive web-based tool, providing a dynamic way for users to explore abstract clusters and examine the topics within each group.

Despite its innovative approach, the study also encountered challenges. One notable limitation was the complexity involved in optimizing the clustering parameters, such as the dimensionality of the embeddings and the number of clusters generated. The reliance on abstract text alone posed another challenge, as abstracts may not fully capture the depth and complexity of the research presented in the corresponding publications. Additionally, some clusters contained outliers or a minimal number of documents, which could skew the accuracy and representation of the topics. Nevertheless, the article demonstrates the potential of transformer-based models in facilitating a more nuanced, unsupervised bibliometric analysis, though it also points to areas where further refinement is needed.

Both articles emphasize the transformative potential of using transformer-based models and large language models in bibliometric analysis, but they also reveal key limitations. The reliance on data quality and availability, the need for optimization of models, and the inherent challenges of working with abstracts or limited datasets are common hurdles faced in the transition from traditional to AI-driven bibliometric approaches.

\begin{description}
    \item[Bibliography Selection and Data Preparation:] In the first step, users select literature based on generic search criteria such as discipline, publication year, and journal name. Data is extracted from academic databases like Scopus, IEEE Xplore, and SerpApi using their respective web services and platforms, or through custom-built web scrapers, such as those powered by SerpAPI. The retrieved data includes bibliographic summaries in CSV format and individual articles in formats like PDF and HTML, which are then stored in a file-based system for further processing.
    \item[Text Embedding and Data Warehousing:] Once the essential documents are retrieved, a Python script leveraging the PyPDF2 library is used to parse the bibliographic summaries, which include the list of downloaded articles along with supportive metadata (e.g., authors, year, source, citations, and h-index), as well as the PDF and HTML versions of the individual articles. This parsing process is designed to upload key textual information into a datastore, building the knowledge base for the proposed AI agent. Unlike traditional information and content management systems, our workflow utilizes a sentence transformer, specifically the all-MiniLM-L6-v2 model from Hugging Face, to generate text embeddings—vector representations that encode the semantic and contextual meaning of the text. These embeddings facilitate more efficient semantic and contextual searches in later stages of the workflow. The text embeddings, along with essential metadata and article content, are uploaded into the datastore. We selected Neo4j, a graph database, as the datastore for this workflow due to its graph data model, which better represents the relationships between data entities stored as nodes in the database. In our project, individual articles are represented as nodes within Neo4j, with associated metadata, content, and text embeddings stored as properties of each node.
    \item[Semantic and Contextual Search]: In the third step, the workflow enables semantic and contextual search of the literature stored in the knowledge (implemented using neo4j database and sentence transformers) based on users' query texts that are collected through a chatbot interface. The core feature of the advanced search relies on the principle of comparing the article's text embedding between the user query texts and the article contents. We employed an enhanced cosine similarity analysis that calculate a numerical similarity score with the range from 0 to 1 to characterize the relevance of of the article based on the users' query, with 0 being completely irrelevant and 1 being highly relevant. The cosine similarity analysis is repeated for all the article stored in the database, with the similarity score calculated for individual article. T 
    \item[]
\end{description}


SentenceTransformer: When used in the context of the SentenceTransformer framework, this model is fine-tuned for producing sentence embeddings rather than performing MLM or CLM tasks directly. The goal is to generate a single dense vector that represents the meaning of the entire sentence, which can be used for tasks like sentence similarity, clustering, and semantic search. This fine-tuning usually involves tasks like Natural Language Inference (NLI) or paraphrase identification rather than MLM or CLM.


 
\begin{enumerate}
    \item What is the nature of the research methodology? Select one or more options from the following categories: "simulation," "data analytics," "experiment," "not applicable."
    \item What is the spatial scale of this research? Choose from the following categories: "global," "national," "state," "multiple cities," "single city," "not applicable."
    \item Does the research use open and public data? Answer using the following categories: "yes," "no," "not specified."    
    \item What is the nature of the contribution? Select from the following categories: "science," "technology," "application," "review," "not applicable."
    \item List all datasets used in this research as an array.
    \item Does the research involve any of the following aspects? Choose one or more options: "social," "policy," "demographic," "economics."   
\end{enumerate}

